Matching Patterns with Variables Under Simon's Congruence

We introduce and investigate a series of matching problems for patterns with variables under Simon's congruence. Our results provide a thorough picture of these problems' computational complexity.

==> poly_algorithm.tex <==
\todo[inline]{As the problems considered in this (sub)section are solved by previous P remarks
(which are waaay shorter), the approach used here can probably be removed, right?}

\todo[inline]{Maybe some parts can be moved to the appendix, let's see.}

By fixing the alphabet to a constant size, we can use an adapted version the universality signatures introduced before
to get a polynomial time complexity algorithm to decide whether for a 1-Var pattern $\psi$ there
exists a substitution $h$ such that $\iota(h(\Psi))=k$ for some universality index $k$.

As we consider only 1-Var patterns in this case, we only consider valid substitutions for one variable.
Before, we guessed a valid signature to get $\NP$-containment. Now, we try all possible signatures to
reach a valid one (if it exists). As the size of the alphabet is fixed to a constant $\sigma$,
we get a polynomial dependency on an input pattern $\psi$ and a universality index $k$.

Algorithm \ref{alg:1-var-subsitution-existence-checker} contains the main method of trying all
signatures and checking whether we reach the valid universality index $k$.
It starts by checking the edge cases such that $\iota(h(X))=0$ for a substitution $h$ on a pattern $\psi$. 
Then, it iterates through all possible signatures for words with an universality index
up to $k$. For each one, first, it checks whether the signature is valid and, second, if it is,
uses Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} to calculate the current
universality index and returns true if it is $k$.

Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} contains the procedure of
calculating the universality index $k$ for a given pattern $\psi$ and an adapted substitution 
signature $(\gamma,p,\delta,R_1,...,R_{\sigma})$.
We start by showing that Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} provides
the correct universality index.

\begin{lemma}\label{lemma:proof-alg-calculator}
    Given a 1-Var pattern $\psi$ and adapted signature $S = (\gamma,p,\delta,R_1,\cdots,R_\sigma)$ for which
    we know that a word $v$ exists.
    For all substitutions $h$ such that $h(X)$ has signature $S$
    we have $\iota(h(\psi))=k$ if and only if Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} returns $k$.
\end{lemma}
\begin{proof}
    Let $\psi$ be a 1-Var pattern and $S = (\gamma,p,\delta,R_1,\cdots,R_\sigma)$ an adapted signature for
    which we know that a word $v$ exists such that $v$ has signature $S$.
    Let $u_1,...u_{n+1}\in\Sigma^*$ such that $\psi=u_1Xu_2...u_nXu_{n+1}$
    
    Let $h$ be a substitution such that $h(X)$ has signature $S$ and $\iota(h(\psi))=k$.
    We can calculate $k$ by iteration over the factors $u_i$ of $\psi$.
    If $i=1$, then there exists so prefix. Let $\iota(u_1)=k_1$.
    We get $\iota(h(\psi)) = k_1 + k_1' = k$ for some number $k_1'$.
    After that, as $h(X)$ has signature $S$, we can calculate $\iota(u_1X)$ using $S$.
    Consider $re(u_1)$. Iterate through $\gamma$ in $S$ and store every letter in a word $s_1$ until
    we reach the first letter such that $\iota(re(u_1)s_1=1$. Then, check whether the last considered index
    in $\gamma$ is smaller or larger than $\delta$ in $S$. If it is smaller or equal to $\delta$,
    we know $\iota(re(u_1)h(X))= 1 + p$. Otherwise we know that we have $\iota(re(u_1)h(X))= 1 + p - 1 = p$
    Call that value $\iota(re(u_1)h(X)) = k_{x1}$.
    Then, we get $\iota(u_1h(X))=k_1 + k_{x1} + k_{x1}'$ for some number $k_{x1}'$.
    Let $j$ be the last checked index in $\gamma$. Let $r_1\in R_j$ be a word such that it is a permutation of the letters
    in $R_j$. Then we also know that $k_{x1}' = \iota(r_1u_2Xu_3...u_nXu_{n+1})$.
    Now, inductively calculate $\iota(r_1u_2Xu_3...u_nXu_{n+1})$ by, first, considering $\iota(r_iu_{i+1})$
    and then considering $\iota(re(r_iu_{i+1})h(X))$ which we calculate as we did before. Also determine $r_{i+1}$
    as we did before. Once we reach $u_{n+1}$, we only have to calculate $\iota(r_{n}u_{n*1})$ and are done.
    We get $k = k_1 + k_{x1} + k_2 + ... + k_n + k_{xn} + k_{n+1}$ such that each $k_1$ and $k_{xi}$ is calculated
    the way we did before. 

    This is the exact calculation performed in Algorithm \ref{alg:1-var-pattern-signature-universality-calculator}.
    First, we factorize $\psi$ such that $\psi=u_1Xu_2 ... u_nXu_{n+1}$. Then we iterate over all factors 
    $u_i$. If $i=1$, we only consider $\iota(u_1) + \iota(re(u_1)h(X))$ and determine the rest $r_1$. 
    If $1 < i < n+1$, we add the values of $\iota(r_{i-1}u_i)$ and $\iota(re(r_{i-1}u_i)h(X))$ and determine the rest
    $r_i$. And if $i = n+1$, we add the value of $\iota(r_nu_{n+1})$.

    As the algorithm performs the same calculation over the same factorization we made in the proof,
    we know that the algorithm is correct and sound for all $\psi$ and $S = (\gamma,p,\delta,R_1,\cdots,R_\sigma)$
    such that $h(X)$ has signature $S$ for all $h$ with $\iota(h(\psi))=k$.
\end{proof}

% MAIN ALGORITHM: Try all signatures
\begin{algorithm}[H]
\caption{Decide Existence of $h$ such that $\iota(h(\psi))=k$ for an alphabet of constant size $\sigma$}\label{alg:1-var-subsitution-existence-checker}
\begin{algorithmic}[1]
\Require 1-Var pattern $\psi$, $X\in\tt{var}(\psi)$, number $k$
\Ensure \emph{True} if substitution $h$ such that $\iota(h(\psi))=k$ exists, otherwise \emph{false.}
\For{$v\in\Sigma^*$ with $\iota(v)=0$ and $\forall\tt{a}\in\Sigma : |v|_{\tt{a}}\leq2$}
    \State Set substitution $h$ such that $h(X)=v$;
    \If{$\iota(h(\psi)) = k$} 
        \State return \emph{true};
    \EndIf
\EndFor
\For{permutation $\gamma$ of $\Sigma$} \Comment{Iterate through all possible Signatures}
    \For{$p \gets 0$ to $k$}
        \For{If $p \neq 0$ then $\delta = 1$ to $3$ otherwise $\delta=3$}
            \For{$R_1 \subset \Sigma$}
                \For{$\cdots$}
                    \For{$R_{\sigma} \subseteq R_{\sigma-1}$} \Comment{Per Signature, check $\iota(h(\psi))=k$}
                        \If{Signature $(\gamma,p,\delta,R_1,...,R_{\sigma})$ is valid}
                            \State Determine universality $\iota(h(\psi))=k_{total}$ for pattern 
                            \State and substitution signature $(\gamma,p,\delta,R_1,...,R_{\sigma})$;
                            \If{$k_{total} = k$}
                                \State return \emph{true};
                            \EndIf
                        \EndIf
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
\EndFor
\State return \emph{false};
\end{algorithmic}
\end{algorithm}

% SECOND ALGORITHM: Calculate k for a given signature
\begin{algorithm}[H]
\caption{Determine $\iota(h(\psi)$ for pattern $\psi$ and substitution signature under an alphabet of constant size $\sigma$}\label{alg:1-var-pattern-signature-universality-calculator}
\begin{algorithmic}[1]
\Require 1-Var pattern $\psi$, substitution signature $(\gamma,p,\delta,S_1,\cdots,S_{\sigma})$
\Ensure Return $k$ such that $\iota(h(\psi))=k$ for all valid substitutions $h$ regarding signature.

\State Factorize $\psi = u_1Xu_2\cdots u_nXu_{n+1}$ for some $u_1,..,u_{n+1}\in\Sigma^*$
\State Set $k_{total} \gets 0$, $re_{current}$ $\gets \emptyset$;
\For{$i = 1$ to $n+1$}
    \State Set $v\in\Sigma^*$ such that $|v|=|re_{current}|$ and for all
    \State $\tt{a}\in\Sigma^*$ we have $|v|_{\tt{a}}=1$;
    \State Build arch factorization of $vu_i$;
    \State Set $k_{total} \gets k_{total} + \iota(vu_i)$;
    \State Set $re_{current} \gets re(vu_i)$;
    \If{$i < n+1$}
        \For{$j = 1$ to $\sigma$}
            \State $re_{current} = re_{current} \cup \tt{a}_{\gamma(j)}$;
            \If{$\gamma(j) \leq \gamma(\delta)$}
                \State $k_{total} \gets k_{total} + p + 1$;
            \Else
                \State $k_{total} \gets k_{total} + p$;
            \EndIf
            \State $re_{current} \gets S_{\tt{a}_{\gamma(j)}}$;
            \State break;
        \EndFor
    \EndIf
\EndFor
\State return $k_{total}$;
\end{algorithmic}
\end{algorithm}

Having that, we can now show that Algorithm \ref{alg:1-var-subsitution-existence-checker} returns true
if and only if a 1-Var pattern $\psi$ can be substituted to a word $w$ which has a specific universality index $k$.
For that, first, we need to show a helper lemma which allows us to work with the edge cases the way did in
Algorithms \ref{alg:1-var-subsitution-existence-checker}.

\begin{lemma}\label{lemma:iota-0-shortform-1var}
Let $w = u_1vu_2 ... u_nvu_{n+1}$ for some $u_1,u_{n+1},v\in\Sigma^*$ with $\iota(v) = 0$ and
$\iota(w)=k$.
Then, there exists $v'\in\Sigma^*$ such that $\iota(v')=0$, for all $\tt{a}_i\in\Sigma$ we have
$|v'|_{a_i} \leq 2$, and $\iota(u_1v'u_2 ... u_n v' u_{n+1}) = \iota(w) = k$.
\end{lemma}
\begin{proof}
Let $w = u_1vu_2 ... u_nvu_{n+1}$ for some $u_1,u_{n+1},v\in\Sigma^*$ with $\iota(v) = 0$ and
$\iota(w)=k$.
Pick $i$ such that $v[i]=\tt{a}_j$ is the first occurrence of the last letter $\tt{a}_j$ in $v$.
Then $\tt{alph}(v[1...i-1]) = \tt{alph}(v)\setminus\{\tt{a}_j\}$.
Let $v_1'\in\Sigma^*$ such that $|v_1'|=|\tt{alph}(v[1...i-1])|$ and for all $\tt{a}_k\in\tt{alph}(v[1...i-1])$ we have
$|v_1'|_{\tt{a}_k}=1$.
Let $v_2'\in\Sigma^*$ such that $|v_2'|=|\tt{alph}(v[i+1...|v|])|$ and for all $\tt{a}_k\in\tt{alph}(v[i+1...|v|])$ we have
$|v_2'|_{\tt{a}_k}=1$.
Let $v' = v_1'v_2'$.
Let $v' = v_1'v_2'$. Then, we see that $\iota(u_1v'u_2...u_nv'u_{n+1})=\iota(u_1vu_2...u_nvu_{n+1})=k$ as the modus of 
both words is the same and the body of each arch $ar_i$ contains the same letters in each word.
\end{proof}

\begin{remark}
In particular, by Lemma \ref{lemma:iota-0-shortform-1var}, we get the same result for words $w$ with one occurrence of such
a factor $v\in\Sigma^*$ with $\iota(v)=0$ such that $w = u_{\ell}vu_r$ for some $u_{\ell}vu_r$.
\end{remark}

With that, we can now show the correctness and soundness of Algorithm \ref{alg:1-var-subsitution-existence-checker}.

\begin{lemma}\label{lemma:proof-alg-checker}
    Given a 1-Var pattern $\psi$, a fixed alphabet of size $\sigma$ and a 
    number $k\in\mathbb{N}$, there exists a substitution $h$ such that $\iota(h(\psi))=k$,
    if and only if Algorithm \ref{alg:1-var-subsitution-existence-checker} returns \emph{true}.
\end{lemma}
\begin{proof}
    Let $\psi$ be a 1-Var pattern and $k$ a number.
    
    \textbf{($\Leftarrow$)}: Assume Algorithm \ref{alg:1-var-subsitution-existence-checker} returns true.
    If Algorithm \ref{alg:1-var-subsitution-existence-checker} returned true  in the first for loop,
    then we found a word $v$ such that there exists a substitution $h$ with $h(X)=v$ and $\iota(h(\psi))=k$.
    The claim follows immediately by that.
    Otherwise, Algorithm \ref{alg:1-var-subsitution-existence-checker} returned true for a signature
    $(\gamma,p,\delta,R_1,...,R_{\sigma})$. By Lemma \ref{lemma:proof-alg-calculator} and
    [BY CHECK ALGORITHM] 
    we know that there exists a substitution $h$ such that $\iota(h(\psi))=k$. This concludes this direction of the proof.

    \textbf{($\Rightarrow$)}: Assume there exists a substitution $h$ such that $\iota(h(\psi))=k$.
    
    \emph{Case 1:} $h(X)=v$ for some $v\in\Sigma^*$ such that $\tt{alph}(v)\subset\Sigma$.
    Then, $h(\psi) = u_1vu_2...u_n v u_{n+1}$. Now, by Lemma \ref{lemma:iota-0-shortform-1var} there exists
    a word $v'\in\Sigma^*$ such that $\iota(v')=0$, for all $\tt{a}_i\in\Sigma$ we have
    $|v'|_{a_i} \leq 2$, and $\iota(u_1v'u_2 ... u_n v' u_{n+1}) = \iota(h(\psi)) = k$.
    By that we know that Algorithm \ref{alg:1-var-subsitution-existence-checker} finds such a word in its
    first for loop and returns true.
    
    \emph{Case 2:} Let $u = h(X)$ for the variable $X$ in $\psi$ such that $\iota(v)>0$. 
    Let $S = (\gamma,p,\delta,R_1,...,R_{\sigma})$ be the adapted universality signature of $u$. 
    Then, as Algorithm \ref{alg:1-var-subsitution-existence-checker} iterates through all possible 
    adapted universality signatures of $u$, we eventually get $S$.
    As $\iota(h(\psi))=k$, Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} will return
    $k$ for $\psi$ and $S$. Therefore, Algorithm \ref{alg:1-var-subsitution-existence-checker} will return true.

    This concludes this proof.
\end{proof}

Having shown that the algorithms are correct and sound, we now show the polynomial time complexity.
First, we show that Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} runs in linear
time complexity if the alphabet is fixed to a constant size.

\begin{lemma}\label{lemma:runtime-algorithm-calculate}
    Given a 1-Var pattern $\psi$ and an adapted universality signature $S = (\gamma,p,\delta,R_1,\cdots,R_\sigma)$.
    Let $\sigma$ be the size of an alphabet with constant size. Then,
    algorithm \ref{alg:1-var-pattern-signature-universality-calculator} has a time complexity of $O(|\psi|)$.
\end{lemma}
\begin{proof}
    Algorithm \ref{alg:1-var-pattern-signature-universality-calculator} starts by factorizing $\psi$
    in factors $u_i$ containing only terminal letters and its variables. This can be done in linear time by
    iterating over the symbols in $\psi$ ($O(|psi|)$).
    Then we iterate over each factor $u_i$.
    For each such factor $u_i$, we build the arch factorization of that factor.
    This can the done in linear time dependent on the size of the factor $u_i$.
    Then, we incorporate the given adapted signature $S$ of the variable substitution,
    if after $u_i$ follows a variable in the pattern.
    For each such incorporation we iterate at max over all letters of the alphabet to determine the considered rest $R_j$
    for the next iteration and the amount of arches $k_{local}$ to add. As the alphabet is sized to a constant
    bound $\sigma$, this takes $O(\sigma)=O(1)$ time.
    Eventually, we iterated over all factors $u_i$ once and did the incorporation of the signature $n$ times.
    This results in an amortised time complexity of $O(|\psi|+|\psi|\cdot\sigma)$ which is equal to $O(|\psi|)$
    if $\sigma$ is bound by a constant factor.
\end{proof}

With that, we immedietely get the time complexity of Algorithm \ref{alg:1-var-subsitution-existence-checker}.

\begin{lemma}
    Given a 1-Var pattern $\psi$ and a number $k\in\mathbb{N}$,
    Algorithm \ref{alg:1-var-pattern-signature-universality-calculator}
    has a time complexity of O($k^2 \cdot |\psi|$) if the size of the alphabet is fixed to a constant size $\sigma$.
\end{lemma}
\begin{proof}
    Algorithm \ref{alg:1-var-subsitution-existence-checker} is divided in two parts.
    The first part checks for all edge cases such that $h(X)=v$ if $\iota(h(\psi)) = k$, for some substituted word
    $v$ with $\iota(v)=0$ and for all letters $\tt{a}\in\Sigma$ we have $|v|_{\tt{a}}\leq2$. 
    For that, we build all possible words up two length $|v| = 2(\sigma-1)$ with the above leeter constraint.
    One upper bound of that is the number of permutations of all words up to length $2(\sigma-1)$
    which results in a number of $2(\sigma-1)!$ many iterations. Per iteration we check whether the
    selected substitution $h$ yields a valid universality index $k$ for $h(\psi)$. This check takes
    linear time in dependency on the length of $\psi$ and the size of the substitution which is bounded by
    a constant factor. So, as $\sigma$is bounded by a constant factor we get a total time complexity of
    $O(|\psi|)$ for this part.

    The second part iterates through all possible adapted universality signatures such that they refer to
    substitutions with a universality up to length $k$. For each such signature $S$, 
    Algorithm \ref{alg:1-var-subsitution-existence-checker} calls Algorithm \ref{alg:1-var-pattern-signature-universality-calculator}
    in order to calculate whether $S$ yields a substitution $h$ such that $\iota(h{\psi})=k$.
    The amount of considered adapted signatures is bound by the choice of its contained values.
    By looking at the \emph{for-loops} we get an upper bound of $\sigma!\cdot k\cdot \sigma \cdot 2^{\sigma^{\sigma}}$.
    As $\sigma$ is bound by a constant factor, this collapses to a runtime complexity of $O(k)$.
    By Lemma \ref{lemma:runtime-algorithm-calculate} we know that Algorithm \ref{alg:1-var-pattern-signature-universality-calculator}
    has a time complexity of $O(|\psi|)$.
    So, in total, we get that Algorithm \ref{alg:1-var-subsitution-existence-checker} has a time complexity of
    $O(k \cdot |\psi|)$.
\end{proof}

\noindent By that we have shown that we can solve our problem for a certain sub-class of patterns in polynomial time.
We reached that complexity bound by considering an alphabet of constant size and by using universality
signatures as a way of describing substitutions that yield words of a very specific structure and universality. \\

This approach is extendable to multiple variables. As adding more variables increases the complexity
exponentially, however, we need to fix them to a constant amount beforehand, too.
On the other hand, the amount of occurrences of a single variable is not that significant regarding the
complexity, as a single signature for a single variable describes the substitutions of all occurrences of
that variable. It will only increase the length of the substituted words in the edge cases of Algorithm 
\ref{alg:1-var-subsitution-existence-checker}. This, however, is still in $P$.

\subsection{Special Case: Any pattern with a variable which only occurs once}

If $\psi$ is any pattern such that there exists a variable which only occurs once in that
pattern, we get a similar complexity to solve the problem as we have in the case of any 1-Var
pattern.

By setting all other variables to the empty word, we basically get a 1-Var pattern with only
once occurrence of a single variable. As the terminal letters in the rest of the word are
fixed, the lower universality index bound is determined by the universality of only the
terminal projection. So it is sufficient, to consider the singular occurring variable and
applying Algorithm \ref{alg:1-var-subsitution-existence-checker} to determine whether we
find a valid substitution $h$ for $\psi$ such that $\iota(h(\psi))=k$ for any $k$.

\todo[inline]{As the problems considered in this (sub)section are solved by previous P remarks
(which are waaay shorter), the approach used here can probably be removed, right?}
